Verifying the correct composition of distributed components: Formalisation and Tool

This article provides formal definitions characterizing well-formed composition of components in order to guarantee their safe deployment and execution. Our work focuses on the structural aspects of component composition; it puts together most of the concepts common to many component models, but never formalized as a whole. Our formalization characterizes correct component architectures made of functional and non-functional aspects, both structured as component assemblies. Interceptor chains can be used for a safe and controlled interaction between the two aspects. Our well-formed components guarantee a set of properties ensuring that the deployed component system has a correct architecture and can run safely. Finally, those definitions constitute the formal basis for our Eclipse-based environment for the development and specification of component-based applications.

==> eptcsdata.tex <==
\providecommand{\firstpage}{69}
\providecommand{\publicationstatus}{Javier C\'amara and Jos\'e Proen\c{c}a (Eds.):\\
13th International Workshop on Foundations of\\
Coordination Languages and Self-Adaptive Systems (FOCLASA'14)\\
EPTCS 175, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.175.5}{10.4204/EPTCS.175.5}}
\pdfoutput=1

